Sensor-Based Safety-Critical Control Using an Incremental Control Barrier Function Formulation via Reduced-Order Approximate Models

The existing control barrier function literature generally relies on precise mathematical models to guarantee system safety, limiting their applicability in scenarios with parametric uncertainties. While incremental control techniques have shown promise in addressing model uncertainties in flight control applications, translating these approaches to safety-critical control presents significant challenges. This paper bridges this gap by introducing measurement-robust incremental control barrier functions (MRICBFs), which leverage sensor-based reduced-order models to provide formal safety guarantees for uncertain systems. By carefully addressing the challenges of sensor accuracy and approximation errors in the incremental formulation, our approach enables substituting specific model components with real-time sensor measurements while maintaining rigorous safety guarantees. This formulation overcomes the limitations of traditional adaptive control methods that adjust system parameters over time, enabling immediate and reliable safety measures for a class of model uncertainties. The efficacy of MRICBFs is demonstrated in two simulation case studies: a simple first-order system with time-varying sensor biases and a more complex overactuated hypersonic glide vehicle with multiple state constraints.

==> Sections/Problem_Formulation.tex <==
We consider a modified version of the nonlinear model, described in Eq. \eqref{NonlinearPlant}, with multiplicative uncertainties on the non-control-related system dynamics of the form:
\begin{equation}
\dot{x} = \Lambda f(x) + g(x)u
\end{equation}
\begin{equation}
\label{ModelProlem}
y = h(x),
\end{equation}
\brownc{Johannes: I decided to consider that problem to state the problem in a simple way. Since $\lambda_i$ can be any value, it still has the implication that the first term is more or less unknown. However, I didn't add uncertainties on $g(x)$ because it would lead to some problem in the boundary area and would lose guarantees.}
where $\Lambda\in \mathbb{R}^{n \times n}$ is a diagonal matrix with $\lambda_i \in \mathbb{R}$ and $\forall i \in [1,n]$ unknown entries:
\begin{equation}
\Lambda = 
\begin{bmatrix}
\lambda_1       & \ldots        & 0 \\
\vdots          & \ddots        & \vdots \\
0               & \ldots        & \lambda_n  
\end{bmatrix}
\end{equation}
The control objective is to determine a $u$ for \eqref{LinearPlantModel} such that the plant state $x_p$ tracks a desired reference $ x_d$ and that for any initial condition $x_0 := x(t_0) \in S$, it is ensured that the plant state vector $x_p$ stays within the safe set $S \subset \mathbb{R}^n$ i.e. the control input ensures that there is a CBF with $h(x) \geq 0$ for all $t \geq 0$.

%Overall, the problem statement here is that we would like to determine a control input $u$ in \eqref{LinearPlantModel} that  guarantees (i) stability, (ii) safety, and (iii) performance in the form of tracking when the matrix $\Lambda$ is unknown and when the control input is restricted in magnitude.


==> Sections/RICBF.tex <==
In the previous section, it was concluded that the condition \eqref{Incremental_Control_Barrier_Function} stated in Theorem \ref{theorem_ICBF} is challenging to satisfy by a controller since the terms $\delta(z, x_0, u_0)$ and $e(x_0, \dot{x}_0)$ are unknown. However, it is possible to formulate bounds on these error terms, leading to a robust controller formulation capable of handling certain aspects of the unknown dynamics, in the following section introduced as robust incremental control barrier functions (RICBFs). Without a loss of generalization, we can assume that the unknown error function $e(x_0, \dot{x}_0)$ of the state derivative measurement lies within a compact error set $E(x_0, \dot{x}_0)$, bounding the measurement uncertainty \cite{Cosner2021}. This leads to the formulation of a maximum error norm, denoted as
\begin{equation}
\label{bound_measurement_error}
\epsilon = \max_{e \in E(x_0, \dot{x}_0)} \|e(x_0, \dot{x}_0)\|_2.
\end{equation}
In a conservative way, we assume that 
\begin{equation}
\label{bound_measurement_error_upper_lower}
-\epsilon \leq e(x_0, \dot{x}_0) \leq + \epsilon.
\end{equation}
Next, we consider the truncation error function. The norm of the truncation error is given by
\begin{equation}
    \|\delta(x, \Delta t)\| = \|A_0 \Delta x + \mathcal{O}(\Delta x^2)\|,
\end{equation}
where \( \Delta x \approx \dot{x} \Delta t \). As $\Delta t \to 0$, the truncation error diminishes, i.e.,
\begin{equation}
    \lim_{\Delta t \to 0} \|\delta(x, \Delta t)\| = 0.
\end{equation}
This indicates that the truncation error becomes negligible for sufficiently high sampling frequencies. Furthermore, as discussed in \cite{Wang2022}, the norm of the error suggests that for any truncation error $\delta > 0$, there exists a $\Delta t > 0$ such that for all $0 < \Delta t < \overline{\Delta t}$,
\begin{equation}
    \|\delta(z, \Delta t)\| \leq \overline{\delta}_e.
\end{equation}
leading to the following conservative assumption that 
\begin{equation}
\label{bound_measurement_error_upper_lower}
-\overline{\delta}_e \leq \delta(z, x_0, u_0)\leq \overline{\delta}_e.
\end{equation}

With these error bounds in place, we can design controllers that ensure the provable safety of incremental CBFs even in the presence of bounded uncertainties.

\begin{theorem}
\label{theorem_RICBF}
Given a set $S \subset \chi$, defined via the associated RICBF, any Lipschitz continuous incremental controller $k(x) \in K_{RIS}$, with 
\begin{equation*}
    K_{RIS}(x) = \{ \Delta u \in \Omega : \dot{h}( \hat{\dot{x}}_0, x_0, u_0, \Delta u) \geq -\alpha(h(x)) \},
\end{equation*}
where
\begin{equation*}
\dot{h}( \dot{x}_0, x_0, u_0, \Delta u) =\frac{\partial h}{\partial x}
\begin{bmatrix} 
\hat{\dot{x}}_0 + g(x_0) \Delta u - \overline{\delta}_e - \epsilon \end{bmatrix}
\end{equation*}
renders the system \eqref{NonlinearPlant} forward invariant within $S$.
\end{theorem}
%%%%%
%%%%
%%%%
\begin{proof}
We again consider exclusively the conditions on the boundary of the safe set $\partial S$ to proof Nagumo's theorem to guarantee forward invariance. We consider the following Lipschitz continuous min-norm controller
\begin{argmini*}
    {\Delta u^* \in \Omega}{\| \Delta u^*\|_2^2}
    {}{}
    \addConstraint{\\ &\frac{\partial h}{\partial x}
\begin{bmatrix} 
\hat{\dot{x}}_0 + g(x_0) \Delta u - \overline{\delta}_e - \epsilon \end{bmatrix} \geq -\alpha(h(x)) }.
\end{argmini*}
The KKT conditions provide us with the following control law:
\[
\Delta u^*(x) =
\begin{cases}
0, & \text{if }\quad B(x) = 0, \\
- \frac{A(x) + \Theta(z, x_0, u_0)}{B(x)^T B(x)} B(x), & \text{if } \quad B(x) \neq 0.
\end{cases}
\]
with $A(x) = \frac{\partial h}{\partial x} \left( \hat{\dot{x}}_0 \right)$, $B(x) = \frac{\partial h}{\partial x} \left( g(x_0)\right)$ and $\Theta(x) = \frac{\partial h}{\partial x} \left( \overline{\delta}_e + \epsilon \right)$. Substitution into the left-hand side of the constraint in \eqref{definition_incremental_safe_controller} leads again to two distinct cases. Case 1 \( B(x) = 0 \): \(A(x)\) must be sufficiently large to counteract the possible worst-case values of \(-\frac{\partial h}{\partial x} \overline{\delta}_e\) and \(-\frac{\partial h}{\partial x} \epsilon\). Case 2 \( B(x) \neq 0 \): At $x \in \partial S$ the control law $\Delta u^*(x)$ leads to:
\[
\dot{h}(x) = (1-\kappa)\delta_{\text{bar}} + (1-\lambda)\epsilon.
\]
with \(\delta(z, x_0, u_0) = -\kappa\delta_{\text{bar}}\) where \(0 \leq \kappa \leq 1\) and \(e(x_0, \dot{x_0}) = -\lambda\epsilon\) where \(0 \leq \lambda \leq 1\). It is easy to see that the controller covers the worst case $\kappa = \lambda = 1$ by ensuring $\dot{h}(x) = 0$ and for cases in which $\kappa, \lambda < 1$ that $\dot{h}(x) > 0$ satisfying Nagumo's theorem.

